Climate of the Field: Snowmass 2021

How are formal policies put in place to create an inclusive, equitable, safe environment? How do these differ between different communities of practice (institutions, labs, collaborations, working groups)? What policies towards a more equitable community are working? For those that aren't working, what external support is needed in order to make them more effective? We present a discussion of the current climate of the field in high energy particle physics and astrophysics (HEPA), as well as current efforts toward making the community a more diverse, inclusive, and equitable environment. We also present issues facing both institutions and HEPA collaborations, with a set of interviews with a selection of HEPA collaboration DEI leaders. We encourage the HEPA community and the institutions & agencies that support it to think critically about the prioritization of people in HEPA over the coming decade, and what resources and policies need to be in place in order to protect and elevate minoritized populations within the HEPA community.

==> AdditionalResources.tex <==
\newcommand{\link}[1]{\href{#1}{link}}
% \section{Misc References} 
% \subsubsection{Codes of Conduct}
% \begin{itemize}
% \item Instituto Nazionale di Fisica Nucleare (INFN) (\link{https://home.infn.it/images/cug/Codice_Etico_INFN_EN.pdf})
%     \item NOvA (\link{https://drive.google.com/file/d/14BjLJ6ezCtdXmdlPPTjbYJ28dthA-UsF/view?usp=sharing}), which draws heavily from LSST/DESC (\link{https://lsstdesc.org/assets/pdf/policies/LSST_DESC_Professional_Conduct.pdf})
%     \item nEXO (\link{https://nexo.llnl.gov/diversity-equity-and-inclusion})
%     \item American Physical Society (APS) Meetings (\link{https://www.aps.org/meetings/policies/code-conduct.cfm})
%     \item American Astronomical Society (AAS)  (\link{https://aas.org/policies/ethics})
% \end{itemize}


% \subsubsection{Climate Statements}
% \begin{itemize}
%     \item Wright Laboratory @ Yale (old statement: \link{https://drive.google.com/file/d/17RkY60iNyQICEi2NqOlc-Q1xIApk9Wk0/view?usp=sharing}, now merged with Yale Physics)
%     \item LIGO scientific collaboration (\link{https://dcc.ligo.org/LIGO-M1400285/public})
%     \item American Institute of Physics (AIP) Diversity Statement (\link{https://www.aip.org/diversity-initiatives/diversity-statement})
% \end{itemize}


\subsection*{Diversity and Inclusion Publications / Presentations}
\begin{itemize}
    \item “Diversity Charter of APPEC, ECFA, NuPECC” (\link{http://www.nupecc.org/jenaa/docs/Diversity_Charter_of_APPEC__ECFA__NuPECC-9.pdf})
    \item “Diversity and Inclusion in the CMS Collaboration” (ICHEP 2020) (\link{https://indico.cern.ch/event/868940/contributions/3801003})
    \item “Diversity and Inclusion Activities in the Belle II Collaboration” (ICHEP 2020) (\link{https://indico.cern.ch/event/868940/contributions/3801008/})
    \item "LGBTQ+ Inclusivity in High Energy Physics" (ICHEP 2020) (\link{https://indico.cern.ch/event/868940/contributions/3801005/})
    \item "The Early Career, Gender \& Diversity at LHCb" (ICHEP 2020) (\link{https://indico.cern.ch/event/868940/contributions/3801001/})
    \item "Early Career Initiatives at LHCb" (ICHEP 2020) (\link{https://indico.cern.ch/event/868940/contributions/3801000/})
    \item “Studies related to gender and geographic diversity in the ATLAS Collaboration” (ATL-GEN-PUB-2016-001) (\link{https://cds.cern.ch/record/2202392?ln=en})
    
    \item “An IDEA for Physics Organizations” APS Inclusion, Diversity, and Equity Alliance (APS-IDEA) (\link{https://www.aps.org/programs/innovation/fund/idea-physics.cfm})
    \item “How to Respond to Code of Conduct Reports” (\link{https://files.frameshiftconsulting.com/books/cocguide.pdf})
\end{itemize}



% \subsection{Resources}

\subsection*{Theses}
\begin{itemize}
    \item A Different Kind of Dark Energy: Placing Race and Gender in Physics by Lauren Chambers, Ph.D. (\link{https://laurenmarietta.github.io/pdfs/Chambers_ADifferentKindOfDarkEnergy.pdf})
    \item Gender, Ethnicity, and Physics Education: Understanding How Black Women Build Their Identities as Scientists by Katemari Diogo da Rosa, Ph.D. (\link{https://search.proquest.com/docview/1282654401})
\end{itemize}


\subsection*{Articles}
\begin{itemize}
    \item The 'Benefits' of Black Physics Students by Jedidah C. Isler, Ph.D. (NYT op-ed) (\link{https://www.nytimes.com/2015/12/17/opinion/the-benefits-of-black-physics-students.html})
    \item Disentangling anti-Blackness from physics by Charles D. Brown II, Ph.D. (Physics Today) (\link{https://physicstoday.scitation.org/do/10.1063/PT.6.3.20200720a/full/})
    \item Understanding and Promoting Diversity and Inclusion in Physics (SPS letter from Geraldine Cochran, Ph.D.) (\link{https://www.spsnational.org/the-sps-observer/winter/2017/understanding-and-promoting-diversity-and-inclusion-physics})
    \item The Status of the African-American Physicist in the Department of Energy National Laboratories by Keith H. Jackson, Ph.D. (APS News) (\link{https://www.aps.org/publications/apsnews/200205/backpage.cfm})
\end{itemize}


\subsection*{Funding Resource Documents}
\begin{itemize}
    \item DoE Office of Science: High Energy Physics Advisory Panel (HEPAP), July 2020
    \item Office of Science Diversity, Equity, \& Inclusion Initiatives  (\link{https://science.osti.gov/-/media/hep/hepap/pdf/202007/14-Carruthers-Diversity_Equity_and_Inclusion_in_the_DOE_Office_of_Science.pdf?la=en&hash=C0BF29C74FE960DD64EEC2DB327BEDB09C14816D})
    \item FESAC Report 2020 (\link{https://usfusionandplasmas.org/wp-content/themes/FESAC/FESAC_Report_2020_Powering_the_Future.pdf})
    \item Government-Wide Diversity and Inclusion Strategic Plan 2011 (\link{https://www.opm.gov/policy-data-oversight/diversity-and-inclusion/reports/governmentwidedistrategicplan.pdf})
\end{itemize}

\subsection*{Professional Organizations}
\begin{itemize}
    \item AIP TEAM-UP Full Report (\link{https://www.aip.org/sites/default/files/aipcorp/files/teamup-full-report.pdf})
    \item Inclusive Scientific Meetings Guide (500 Women Scientists) (\link{https://static1.squarespace.com/static/582cce42bebafbfc47a82b04/t/5ca0fe7d9b747a3d7dc7a71f/1554054781756/Formatted+Inclusive+Meeting+Guide-v5.pdf})
    \item LGBT+ Inclusivity in Physics and Astronomy: A Best Practices Guide (\link{https://arxiv.org/pdf/1804.08406.pdf})
    \item NASEM. 2020. The Impacts of Racism and Bias on Black People Pursuing Careers in Science, Engineering, and Medicine: Proceedings of a Workshop. Washington, DC: The National Academies Press. https://doi.org/10.17226/25849. 
    \item NASEM. 2020. Promising Practices for Addressing the Underrepresentation of Women in Science, Engineering, and Medicine: Opening Doors. Washington, DC: The National Academies Press. https://doi.org/10.17226/25585
    % \item Astro Decadal Survey (\link{https://www.nationalacademies.org/our-work/decadal-survey-on-astronomy-and-astrophysics-2020-astro2020}), or more specifically Appendix N (on Equity initiatives) (\link{https://drive.google.com/file/d/1ZyHlBe7wqb-jpFtVBZSVqyNcBQ9Rafuk/view?usp=sharing})
\end{itemize}


% \subsubsection{Public Initiatives}
% \begin{itemize}
%     \item Change-Now Physics: Calls to Action from Black Scientists at Fermilab (\link{https://changenowphysics.com/strategic-plan/})
%     \item \#BlackInAstro stories from astrobites (AAS) (\link{https://astrobites.org/?s=\%23BlackInAstro})
%     \item "How to Respond to Code of Conduct Reports" (\link{https://files.frameshiftconsulting.com/books/cocguide.pdf}) by authors of the Ada Initiative Anti-Harassment framework (\link{https://adainitiative.org/continue-our-work/conference-policies/})


% \end{itemize}


